Stochastic Sparse Sampling: A Framework for Variable-Length Medical Time Series Classification

While the majority of time series classification research has focused on modeling fixed-length sequences, variable-length time series classification (VTSC) remains critical in healthcare, where sequence length may vary among patients and events. To address this challenge, we propose $\textbf{S}$tochastic $\textbf{S}$parse $\textbf{S}$ampling (SSS), a novel VTSC framework developed for medical time series. SSS manages variable-length sequences by sparsely sampling fixed windows to compute local predictions, which are then aggregated and calibrated to form a global prediction. We apply SSS to the task of seizure onset zone (SOZ) localization, a critical VTSC problem requiring identification of seizure-inducing brain regions from variable-length electrophysiological time series. We evaluate our method on the Epilepsy iEEG Multicenter Dataset, a heterogeneous collection of intracranial electroencephalography (iEEG) recordings obtained from four independent medical centers. SSS demonstrates superior performance compared to state-of-the-art (SOTA) baselines across most medical centers, and superior performance on all out-of-distribution (OOD) unseen medical centers. Additionally, SSS naturally provides post-hoc insights into local signal characteristics related to the SOZ, by visualizing temporally averaged local predictions throughout the signal.

==> sections/6acknowledgements.tex <==
\subsubsection*{Author Contributions}


\subsubsection*{Acknowledgements}
Xavier Mootoo is supported by Canada Graduate Scholarships\textemdash Master's (CGS-M) funded by the Natural Sciences and Engineering Research Council (NSERC) of Canada, the Vector Scholarship in Artificial Intelligence, provided through the Vector Institute, Canada, and the Ontario Graduate Scholarship (OGS) granted by the provincial government of Ontario, Canada. We also greatly thank \href{https://communeai.org/}{Commune AI} for generously providing the computational resources needed to carry out our experiments, in particular, we extend our gratitude to Luca Vivona and Sal Vivona. We also thank Anastasios Angelopoulos, for his 


Hina Tabassum is supported through the NSERC Discovery Grant.
